Pneg: Prompt-based Negative Response Generation for Dialogue Response Selection Task

In retrieval-based dialogue systems, a response selection model acts as a ranker to select the most appropriate response among several candidates. However, such selection models tend to rely on context-response content similarity, which makes models vulnerable to adversarial responses that are semantically similar but not relevant to the dialogue context. Recent studies have shown that leveraging these adversarial responses as negative training samples is useful for improving the discriminating power of the selection model. Nevertheless, collecting human-written adversarial responses is expensive, and existing synthesizing methods often have limited scalability. To overcome these limitations, this paper proposes a simple but efficient method for generating adversarial negative responses leveraging a large-scale language model. Experimental results on dialogue selection tasks show that our method outperforms other methods of synthesizing adversarial negative responses. These results suggest that our method can be an effective alternative to human annotators in generating adversarial responses. Our dataset and generation code is available at https://github.com/leenw23/generating-negatives-by-gpt3.

==> 1.Introduction.tex <==
\section{Introduction}
\label{introduction}

In retrieval-based dialogue systems, the response selection model aims to predict the most appropriate response among multiple candidates retrieved for a given conversation context~\citep{zhou-etal-2018-multi, wu2019sequential, chen-etal-2022-contextual}. The selection model is generally trained to distinguish a related (positive) response from randomly sampled negative responses on training datasets, but such a model generally poses the following problems.

\begin{figure}[t]
\centering
\begin{tabular}{c}
     \includegraphics[width=0.48\textwidth]{figures/Pneg.pdf}
\end{tabular}
\caption{A conceptual pipeline of prompt-based negative response generation.}
\label{fig:method}
\vspace{-0.1in}
\end{figure}

First, randomly selected negatives are often too easy to distinguish because they are totally irrelevant to the dialogue context~\citep{li-etal-2019-sampling, lin-etal-2020-world}. In this case, the model is more likely to predict the response only by relying on the superficial content similarity of the context-response pairs~\citep{yuan-etal-2019-multi, sai-etal-2020-improving, whang2021response}. These models are vulnerable to adversarial responses with high content similarity to the dialogue context, and fail to distinguish subtle differences in various contexts in real-world scenarios. Second, random sampling causes sampling bias, such as containing false negatives for a given dialogue context~\citep{zhou-etal-2022-debiased}. These biases inherent in the training datasets hinder the accurate prediction of the selection model, resulting in performance degradation.

To mitigate this problem, recent studies have proposed various methods to synthesize and leverage adversarial negative training samples so that the selection model can learn features beyond content similarity~\citep{srivastava2020robustness, kaushik2021learning}. However, existing methods for synthesizing adversarial negative responses~\citep{ebrahimi-etal-2018-hotflip, alzantot-etal-2018-generating, zhang-etal-2019-generating-fluent, qiu2021challenging, gupta-etal-2021-synthesizing} still have limitations in creating human-like responses. The most reliable method is to collect human-written adversarial negatives~\citep{sai-etal-2020-improving}, but it is not scalable because it is expensive and time consuming.

To overcome these limitations, we note that large-scale language models such as GPT3 can be utilized as a low-cost data labeler~\citep{wang-etal-2021-want-reduce}. In this paper, we present \textsc{Pneg}, a \textbf{P}rompt-based \textbf{NE}gative response \textbf{G}eneration method leveraging a large-scale language model (Figure~\ref{fig:method}). In P-NEG, we can cheaply collect human-like adversarial negatives by using an in-context learning-based data augmentation method with human-written samples as demonstration examples.

Experimental results on the dialogue response selection task show that the selection model that trained the negative samples from \textsc{Pneg} has better performance than other baselines. We then conduct quality evaluation and ablation studies to analyze the validity of \textsc{Pneg}. Consequently, we argue that \textsc{Pneg} can be an efficient alternative to human annotators in generating adversarial responses.

Our contributions are as follows:
\begin{itemize}
    \item We propose \textsc{Pneg}, a \textbf{P}rompt-based \textbf{NE}gative response \textbf{G}eneration method. 
    \item Our method can generate high-quality adversarial negative responses only with a few human-written examples.
    \item We show that our method outperforms other baselines across multiple model architectures on the response selection task.
\end{itemize}


==> 2.Method.tex <==
\section{\textsc{Pneg}: Prompt-based NEgative response Generation}
\label{promptconstruction}
Large-scale language models such as GPT-3~\citep{NEURIPS2020_1457c0d6} can augment fluent text training samples using natural language prompts and in-context examples~\citep{yoo2021gpt3mix, schick-schutze-2021-generating, bae2022building, liu2022wanli}. By extending such direction to the response selection task, we propose \textsc{Pneg}, a \textbf{P}rompt-based \textbf{NE}gative response \textbf{G}eneration method for robust response selection models.
Our method consists of three steps: (1) selecting demonstration examples, (2) constructing a prompt containing examples and target dialogue context, and (3) generating adversarial negative responses by inputting the prompt into GPT-3. The generated negative responses are used as training samples for response selection task.

\begin{figure}[t]
\centering
\begin{tabular}{c}
     \includegraphics[width=0.48\textwidth]{EMNLP 2022/figures/promptConfig.pdf}
\end{tabular}
\caption{Overall pipeline of \textsc{Pneg}.}
\label{fig:promptconfig}
\vspace{-0.1in}
\end{figure}

\subsection{Step 1: Example Selection}
We first sample a total $k$ demonstration examples from an example set $E$ to construct a prompt for in-context learning of GPT-3~(A in Figure~\ref{fig:promptconfig}). We consider \textit{DailyDialog++}~\cite{sai-etal-2020-improving} as an example set to generate training samples that have similar patterns as human-written high-quality linguistic patterns. The example set consists of a dialogue context, a positive response, and multiple human-written negative responses. We uniformly sampled examples from the dialogue dataset. The context and human-written negative responses are used in the following prompt construction step.

\subsection{Step 2: Prompt Construction}
\paragraph{Prompt Design}
We first design a prompt to use as an input to GPT-3. Large-scale language models are generally pre-trained to generate responses with high coherence for a given context, but our method aims to generate adversarial responses with high content similarity but low coherence. In particular, natural language prompt-based reasoning is sensitive to prompt changes~\citep{jin-etal-2022-good}, so we have to carefully design prompts to generate accurate negative responses. We devise several prompts to evaluate generative quality, inspired by related works~\citep{yoo2021gpt3mix, schick-schutze-2021-generating, min2022rethinking}. We evaluate the devised prompts by the response selection task, and then select the finest prompt template based on the results of Appendix~\ref{sec:appendix_prompt_changes}.

\paragraph{Prompt Construction}
Our prompt is constructed with the chosen prompt template, $k$ number of examples, and the target dialogue context that we aim to generate multiple negative responses. The prompt template consists of three components to clarify the role of each example and target context: (1) a task instruction $I$ written in natural language, (2) an enumerator to receive each utterance from examples and the target context, and (3) a separator to separate each example or dialogue context in the prompt. The details of each component in the prompt template are shown in Figure~\ref{fig:promptconfig}.

\subsection{Step 3: Negative Response Generation}
Now, GPT-3 can generates augmented negative responses following our input prompt~(C in Figure~\ref{fig:promptconfig}). The examples within the prompt encourage the language model to generate negative responses of similar patterns to the human-written negative responses. The task instruction directly guides the model to understand the target task and the relationship between a dialogue context and corresponding negative responses in the examples.


==> 3.Experimental_Setup.tex <==
\section{Experimental Setup}
\label{experimental_setup}
\subsection{Dialogue Response Selection Task}
We evaluate our method on the dialogue response selection task. We train the selection model with 11 response candidates consisting of 1 positive response, 5 random and 5 adversarial negative responses per context. We report the R@1 and mean reciprocal rank~(MRR) score. For evaluation, we use random and adversarial test datasets which consist of the 6 candidates for each context.

\subsection{Datasets}
\paragraph{DailyDialog++}
We use the \textit{DailyDialog++}~\cite{sai-etal-2020-improving} dataset for our overall experiments. This dataset consists of 16,900, 1028, and 1142 dialogue contexts in training, validation, and test datasets, respectively. Since only the subset of 9259 contexts in the training dataset contains adversarial responses, we use them as our training dataset. Each context has five adversarially curated negative responses written by human annotators.

\paragraph{PersonaChat}
We also use the \textit{PersonaChat} dataset~\cite{zhang2018personalizing} on the response selection task. This dataset consists of 8938, 1000, and 968 dialogue conversations in training, validation, and test datasets, respectively. We use 8938 contexts for training, and concatenate the persona sentences in front of the context. Since there are no human-written adversarial negative responses in this dataset, we create an adversarial test dataset by sampling one response from the context and including it in the candidate responses following \citet{gupta-etal-2021-synthesizing} and \citet{whang2021response}.

\subsection{Baselines}
\label{baselines}
We compare our method with following baselines.
\paragraph{Random} Randomly sampled responses.
\paragraph{Human~\citep{sai-etal-2020-improving}} Human-written adversarial responses in \textit{DailyDialog++} dataset.
\paragraph{BM25~\citep{karpukhin-etal-2020-dense}} Retrieved responses from BM25~\cite{bm25}.
\paragraph{Semi-hard~\citep{li-etal-2019-sampling}} Retrieved responses from training dataset based on their similarity between positive response with a margin of $\alpha$. We perform a static sampling using sentence-BERT~\cite{reimers-gurevych-2019-sentence} with $\alpha$ as 0.07 following~\citet{gupta-etal-2021-synthesizing}. 
\paragraph{Mask-and-fill~\citep{gupta-etal-2021-synthesizing}} This method first randomly masks the words in a answer response, and infill them using masked language modeling conditioned on a random context.
\paragraph{Key-sem~\citep{gupta-etal-2021-synthesizing}} This method generates new responses conditioned on keywords in the context using GPT-2~\cite{gpt2}.
\paragraph{\textsc{Pneg} (Ours)} GPT-3 generated adversarial negative responses by using our method, \textsc{Pneg}.

\subsection{Models}
\label{Models}
We train dialogue selection models with different negative responses described in \S\ref{baselines}. The models are based on cross-encoder architecture, and three different pre-trained language models are used in experiments: 1) BERT~\cite{devlin2019bert}, 2) RoBERTa~\cite{liu2019roberta}, and 3) ELECTRA~\cite{clark2019electra}. The implementation details are provided in Appendix~\ref{sec:appendix_implementation}.


==> 4.Experiments.tex <==
\section{Experiments}
\label{experiments}
\subsection{Performance on Response Selection Task}
\label{exp:response_selection}
We compare our method with the baselines for the response selection task\footnote{The negative responses samples generated by each method are provided in Table~\ref{table:response_examples}.} (Table~\ref{table:exp1}). On the adversarial test dataset, we notice that \textsc{Pneg} consistently outperforms other baselines across different model architectures. The \textsc{Pneg} especially shows the most similar performance to the human baseline, which suggests that our method can be an effective alternative to human annotators for collecting adversarial negative samples.
In the random test dataset, Semi-hard performs better than other baselines including \textsc{Pneg} and even the human baseline. This tendency indicates that the robustness of the models to the adversarial test dataset does not always lead to the random test dataset.
We speculate that these results are due to data distribution shifts according to different negative response sampling strategies~\citep{penha2021calibration}.
Retrieval-based methods like BM25 and Semi-hard would suffer from finding appropriate negative responses when the dialogue corpus for response retrieval is limited.

We also compare our method with the baselines for the response selection task on the \textit{PersonaChat} (Table~\ref{table:persona}). Although \textsc{Pneg} generates negative responses using human-written examples from \textit{DailyDialog++}, it shows better performance than other baselines in the adversarial test dataset. Such results prove the scalability of \textsc{Pneg} across multiple dialogue datasets, because our method can automatically generate adversarial negative samples with only a few human-written samples. It means that our method can easily transfer to other domain conversations only with minimal human effect. Since we used fewer samples for \textit{PersonaChat} experiments, the response selection models overall show lower performance than the \textit{DailyDialog++} experiment.

\input{0.Main-table}

\input{0.Sub-table}

\subsection{Synthetic Dataset Quality}
\label{synthetic_quality}
We evaluate the quality of adversarial responses with predictive scores of the response selection model and context-response similarity model\footnote{The experiment details are provided in Appendix~\ref{sec:appendix_auto_eval}.}. We assume that the higher the prediction score of the selection model for the adversarial negative response, the more effective it is for the robust training of the model. The evaluation results are shown in Figure~\ref{fig:box_plot}. In both models, the prediction score for negative responses generated by \textsc{Pneg} is higher on average than other responses. The difference is more significant in the score of the selection model, suggesting that \textsc{Pneg} can produce more effective adversarial responses that are confused with the positive response. Although Semi-hard samples negative responses using similarity scores from Sentence-BERT, the responses have lower scores than other methods because the sampling pool is limited. We additionally provide human evaluation results for synthetic quality in Appendix~\ref{exp:human_eval}.

\begin{figure}[t]
\centering
\begin{tabular}{l}
     \includegraphics[width=0.46\textwidth]{figures/box_plot.pdf}
\end{tabular}
\caption{Box plot of prediction scores (blue) and similarity score (orange) for each type of response. The prediction scores are linearly normalized into the [0,1].}
\label{fig:box_plot}
\end{figure}

\subsection{Varying the Size of Example Set}
\label{exp:ablation}
\begin{table}[t]
\centering
    {\small
    {\tabulinesep=0.6mm
    \begin{tabu}{l|c|c|c|c}
    \textbf{Sub. (\%)} & \textbf{$|E|$} & \multicolumn{2}{c|}{\textbf{Test Set (R@1)}} & \textbf{Mean}\\
    \hhline{~|~|--|~|}
    &  & Random & Adv & \scriptsize{Rand + Adv}\\
    \hline
    0.1 +\textsc{reuse} & 9$+\alpha$ & 0.852 & 0.899 & 0.876\\
    0.1 & 9 & 0.843 & 0.938 & 0.891\\
    1 & 93 & 0.845 & 0.936 & 0.891\\
    10 & 926 & 0.852 & 0.936 & 0.894\\
    100 (\textsc{Pneg}) & 9259 & 0.877 & 0.941 & 0.909\\
    \hline
    \end{tabu}
    }}
\caption{\label{table:ex_set} Performance on the size changes of $E$ containing examples used to construct prompts of our method.}
\vspace{-0.1in}
\end{table}
We study the effect of the size of the example set $E$ containing examples for prompt construction on the performance of the response selection task. As shown in Table~\ref{table:ex_set}, even if the size of $E$ becomes extremely small (e.g., 0.1\%), the performance on the adversarial test dataset hardly decreases. These results show that our method can efficiently generate high-quality adversarial responses by collecting only a few demo examples. To increase the diversity of examples, we further try \textsc{+reuse}, which continuously adds the negative responses generated by \textsc{Pneg} to $E$. However, the 0.1\%\textsc{+reuse} has a significant performance drop in the adversarial test dataset. These results shows that example quality is more important than the diversity of examples to optimize the quality of the generated negative responses.


==> 5.Conclusion.tex <==
\section{Conclusion}
\label{conclusion}
In this paper, we present \textsc{Pneg}, a prompt-based adversarial negative response generation method for response selection task. \textsc{Pneg} can collect high-quality adversarial negative responses at a lower cost than human annotators. Our experiments on dialogue response selection tasks show that negative responses generated by \textsc{Pneg} can improve the discriminating power of the selection models. In future work, we are interested in designing more confused adversarial responses and how to effectively utilize them for training the selection models.


==> 6.Limitations.tex <==
\section*{Limitations}
\label{limitations}
In this section, we present two major limitations of our work.
First, \textsc{Pneg} has not yet been tested on a larger dataset. We expect our method can produce effective adversarial training samples in large-scale datasets at a reasonable cost. However, since the performance of sampling-based methods can improve on sufficiently large training datasets, it is necessary to compare such methods with \textsc{Pneg}.
Second, there is a limitation to leveraging the adversarial negative response for training the selection model in the dialogue response selection task. The selection model that learns the adversarial negative response improves performance in the adversarial test dataset with the same distribution of candidates, but decreases performance in the random test dataset. This is not the result we were hoping for, and we need a close analysis to solve this phenomenon.


==> 7.Ethics_Statement.tex <==
\section*{Ethics Statement}
\label{ethics statement}
We clarified compliance with the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL Ethics Policy} in this study. In particular, in the human evaluation experiment, we recruited participants fairly, designed experiments that require minimal effort, and provided adequate rewards to participants.


==> EMNLP 2022/0.Main-table.tex <==
\begin{table}[t]
\centering
    {\small
    {\tabulinesep=0.5mm
    \begin{tabu}{l|l|cc|cc}
    \textbf{Model} & \textbf{Method} & \multicolumn{4}{c}{\textbf{Test Dataset}}\\
    \hhline{~~|----}
    & & \multicolumn{2}{c|}{Random} & \multicolumn{2}{c}{Adversarial}\\
    \hhline{~~|----}
    & & R@1 & MRR & R@1 & MRR\\
    \tabucline[1pt]{-}
    \scriptsize{BERT} & \scriptsize{Random} & 0.865 & 0.923 & 0.674 & 0.806\\
    & \scriptsize{BM25} & 0.845 & 0.911 & \underline{0.857} & 0.915\\
    & \scriptsize{Semi-hard} & \textbf{0.881} & \textbf{0.934} & 0.672 & 0.804\\
    & \scriptsize{Key-sem} & 0.864 & 0.923 & 0.842 & 0.909\\
    & \scriptsize{Mask\&fill} & \underline{0.869} & \underline{0.926} & 0.856 & \underline{0.916}\\
    & \scriptsize{\textsc{Pneg}} & 0.867 & 0.924 & \textbf{0.937} & \textbf{0.964}\\
    \hline
    & \scriptsize{Human} & 0.870 & 0.926 & 0.954 & 0.974\\
    \tabucline[1pt]{-}
    \scriptsize{RoBERTa} & \scriptsize{Random} & 0.879 & 0.932 & 0.658 & 0.797\\
    & \scriptsize{BM25} & 0.879 & 0.932 & 0.865 & 0.920\\
    & \scriptsize{Semi-hard} & \textbf{0.892} & \textbf{0.937} & 0.660 & 0.797\\
    & \scriptsize{Key-sem} & \underline{0.889} & \textbf{0.937} & \underline{0.868} & \underline{0.924}\\
    & \scriptsize{Mask\&fill} & 0.873 & 0.927 & \underline{0.868} & 0.922\\
    & \scriptsize{\textsc{Pneg}} & 0.882 & \underline{0.933} & \textbf{0.942} & \textbf{0.967}\\
    \hline
    & \scriptsize{Human} & 0.891 & 0.938 & 0.955 & 0.975\\
    \tabucline[1pt]{-}
    \scriptsize{ELECTRA} & \scriptsize{Random} & 0.893 & \underline{0.941} & 0.705 & 0.823\\
    & \scriptsize{BM25} & 0.853 & 0.916 & \underline{0.900} & \underline{0.940}\\
    & \scriptsize{Semi-hard} & \textbf{0.908} & \textbf{0.949} & 0.730 & 0.840\\
    & \scriptsize{Key-sem} & \underline{0.895} & 0.940 & 0.869 & 0.929\\
    & \scriptsize{Mask\&fill} & \underline{0.895} & \underline{0.941} & 0.877 & 0.923\\
    & \scriptsize{\textsc{Pneg}} & 0.873 & 0.928 & \textbf{0.951} & \textbf{0.972}\\
    \hline
    & \scriptsize{Human} & 0.896 & 0.941 & 0.967 & 0.982\\
    \tabucline[1pt]{-}
    \end{tabu}}}
    \caption{\label{table:exp1} Performance in the dialogue response selection task on Random and Adversarial test datasets based on the \textit{DailyDialog++}. Among the methods except for human baseline, the best result is shown in \textbf{bold}, and the second-highest result is \underline{underlined}.}
\end{table}


==> EMNLP 2022/0.Sub-table.tex <==
\begin{table}[t]
\centering
    {\small
    {\tabulinesep=0.6mm
    \begin{tabu}{l|c|c|c}
    \textbf{Approach} & \multicolumn{2}{c|}{\textbf{Test Set}} & \textbf{Mean}\\
    \hhline{~|--|~|}
    & Random & Adversarial & Rand + Adv.\\
    \hline
    Random & \textbf{0.815} & 0.316 & 0.566\\
    Semi-hard & \underline{0.814} & 0.338 & 0.576\\
    BM25 & 0.718 & \underline{0.637} & \underline{0.678}\\
    \textsc{Pneg} (Ours) & 0.774 & \textbf{0.684} & \textbf{0.729}\\
    \hline
    \end{tabu}
    }}
    \caption{\label{table:persona} Performance in the dialogue response selection task on Random and Adversarial test datasets based on the \textit{PersonaChat}. Among the methods except for human baseline, the best result is shown in \textbf{bold}, and the second-highest result is \underline{underlined}.}
\vspace{-0.1in}
\end{table}

